Using Spatial Logic and Model Checking for Nevus Segmentation

Spatial and spatio-temporal model checking techniques have a wide range of application domains, among which large scale distributed systems and signal and image analysis. In the latter domain, automatic and semi-automatic contouring in Medical Imaging has shown to be a very promising and versatile application that can greatly facilitate the work of professionals in this domain, while supporting explainability, easy replicability and exchange of medical image analysis methods. In recent work we have applied this model-checking technique to the (3D) contouring of tumours and related oedema in magnetic resonance images of the brain. In the current work we address the contouring of (2D) images of nevi. One of the challenges of treating nevi images is their considerable inhomogeneity in shape, colour, texture and size. To deal with this challenge we use a texture similarity operator, in combination with spatial logic operators. We apply our technique on images of a large public database and compare the results with associated ground truth segmentation provided by domain experts.

==> Statsimil.tex <==
% !TEX root = UIVoxLogica2020.tex 

\section{The \imgqool Operator for Texture Analysis}
\label{sec:LogicTA}

Texture Analysis (TA) is an approach used for finding patterns in (medical) images. 
Such patterns are characterised by distinct combinations of features, such as brightness, colour, shape or size.  
The approach has proved promising in a large number of applications in the field of medical imaging
\cite{Kassner2010,Lopes2011,Castellano2004,Davnall2012}; in particular
it has been used in \emph{Computer Aided Diagnosis}
\cite{Woods2007,Han2014,Heinonen2009} and for classification or
segmentation of tissues or organs
\cite{Chen1989,Sharma2008,RodriguezGutierrez2013}.
%
%In TA, image textures are usually characterised by estimating some
%descriptors in terms of quantitative features. Typically, such
%features fall into three general categories: syntactic, statistical,
%and spectral \cite{Kassner2010}. Our work is mostly focused on
%\emph{statistical} approaches to texture analysis. 
%For two-dimensional images, statistical methods
%consist of extracting a set of statistical \emph{descriptors} from the
%distributions of local features in a neighbourhood of each pixel.
 
In \imgqool a texture analysis operator has been introduced~\cite{BCLM19} that uses \emph{first order} statistical methods. These are statistics based on the probability distribution function of the intensity values of the pixels of parts, or the whole, of an image. 
%The classical first-order statistical approach to TA makes use of 
%statistical indicators of the local distribution of image intensity around each pixel, 
%such as \emph{mean}, \emph{variance}, \emph{skewness}, \emph{kurtosis}, \emph{entropy}
%\cite{Srinivasan2008}.  
%Although such indicators ignore the relative spatial placement of adjacent pixels, 
%statistical operators are useful in MI because their application is invariant under
%transformations of the image, in particular \emph{affine transformations}
%(rotation and scaling), which is necessary when analysing several
%images acquired in different conditions. It is worth mentioning that current research also 
%focuses on constructing features using first order operators, keeping some
%spatial coherence, but loosing at least partially the aforementioned
%invariance \cite{Tijms2011}. 
The TA operator in  \imgqool differs from that in the classical setting, see e.g.~\cite{Srinivasan2008,Tijms2011}. It analyses (the histograms of) statistical distributions directly instead of comparing the various moments (\emph{mean}, \emph{variance} etc.) of the local distribution of image intensity around each pixel. The similarity measure used is the \emph{cross-correlation} function (also called \emph{Pearson's correlation coefficient}).

The idea of the \imgqool texture operator is presented schematically in Figure~\ref{fig:TAsketch}. Suppose we have an SLCS formula $\Phi$ that specifies a sample area of interest in the image. We are looking for pixels that have a local neighbourhood that is similar to that of the sample area $\Phi$. One attribute of pixels that could provide information on this similarity is the intensity of the pixels (but other attributes could be chosen as well, for example their colour). For each pixel $x$ we consider its local neighbourhood and construct a histogram $H_x$ of the intensities of the pixels in this neighbourhood. We also construct a histogram $H_{\Phi}$ of the intensities of the sample area $\Phi$. Then we assign to pixel $x$ the cross-correlation coefficient comparing $H_x$ with $H_{\Phi}$. For that to work, both histograms need to have the same number of bins and the same minimal and maximal values. Once we have obtained the cross-correlation coefficient of each pixel in the image we can easily find all pixels with a sufficiently high score, i.e. those pixels that are sufficiently similar to the sample area. 

\begin{figure}
\centerline{\includegraphics[width=0.45\textwidth]{img/TA_CC_sketch.pdf}}
\caption{\label{fig:TAsketch} Illustration of the texture analysis operator in \imgqool}
\end{figure}  

More formally, the statistical distribution of the values of a numerical attribute in a set of points $Y$ of a space---e.g. the grey levels or intensity of the pixels or voxels of an area of a black and white image---is approximated  by the  \emph{histogram} $h$ of the values of the attribute in the points belonging to $Y$, as described below.

Given a minimum value $m$, a maximum\footnote{The minimum value $m$ and the maximum value $M$ are aimed at improving the resolution of histograms, by excluding rare peaks in the set of points---they might be
due to artefacts in the acquisition in the case of images---and would result in a high
number of empty bins.} value $M$, and a positive number of \emph{bins} $k$, let
$\Delta = (M - m)/k$ and define the histogram $h$ as a function associating to each
\emph{bin} $i \in [1,k]$ the number of points that have the value of the attribute in
the (half-open) interval $[(i-1) \cdot \Delta + m,i \cdot \Delta + m)$. 
 A formal definition  is given below:

\begin{definition}
Given  closure model $\model = ((X,\closure), \aeval, \peval)$,
we define
function $\mkhis : A \times 2^X \times \reals \times \reals \times \nats \to (\nats \to \nats)$
such that for all values $m,M \in \reals$, with $m<M$, and $k,i \in \nats$, with $k>0$ and 
$i\in [1,k]$, letting $\Delta=\frac{M-m}{k}$:\\
$$
\mkhis(a,Y,m,M,k)(i) =
%$%\\
%$
\left|\ZET{y\in Y}{(i-1) \Delta \leq \aeval(y,a) - m < i \Delta}\right|
$$
\ed
\end{definition}
So $\mkhis(a,Y,m,M,k)$ is the histogram of the distribution of the values of attribute $a$ of the points in $Y$, in the interval $[m,M]$ with step size $\Delta$.
%The above definition applies also to quasi-discrete / distance closure models.

The definition of {\em cross correlation} between two histograms follows, where, for histogram $h: [1,k] \to \nats$, we let 
$\mean{h}=\frac{1}{k}\sum_{i=1}^k h(i)$ denote the {\em mean}  of $h$.
\begin{definition}
Let $h_1, h_2: [1,k] \to \nats$ be two histograms. The {\em cross correlation} of
$h_1$ and $h_2$ is defined as follows:
$$
\cc(h_1,h_2) = 
\frac
{\sum_{i=1}^k\left( h_1(i) - \mean{h_1} \right) \left(h_2(i) - \mean{h_2} \right)}
{
\sqrt{ 
\sum_{i=1}^k \left(h_1(i) - \mean{h_1} \right)^2
}
\sqrt{
\sum_{i=1}^k \left(h_2(i) - \mean{h_2} \right)^2
}
}
$$\ed
\end{definition}

The value of $\cc{}{}$ is \emph{normalised} so that
$-1\le \cc(h_1,h_2) \le 1$; $\cc(h_1,h_2)=1$ indicates that $h_1$ and $h_2$
are \emph{perfectly correlated} (that is, $h_1 = ah_2+b$, with $a>0$); $\cc(h_1,h_2) =-1$
indicates \emph{perfect anti-correlation} (that is, $h_1=ah_2+b$, with $a<0$). On the other
hand, $\cc(h_1,h_2) = 0$ indicates no correlation. 

\begin{remark} Note that normalisation
makes the value of $\cc{}{}$ undefined for constant histograms, having
therefore standard deviation of $0$; in terms of statistics, a
variable with such standard deviation is only (perfectly)
correlated to itself. This special case is handled by letting
$\cc(h_1,h_2)=1$ when both histograms are constant, and $\cc(h_1,h_2)=0$ when only one
of the $h_1$ or $h_2$ is constant.
\end{remark}

The statistical similarity operator $\lssim{\bowtie c}{m}{M}{k}{\rho}{a}{b}$ is embedded in  \SLCSMI as follows.

\begin{definition}\label{def:sdsatisfaction}
{\em Satisfaction} $\model, x \models \form$ at point $x \in X$ in model
$\model = (((X,\closure),d), \aeval, \peval)$ is defined by induction on the structure of formulas, by adding the following equation  to those in Figure~\ref{fig:fragSLCSsem}, where $m,M \in \reals$, with $m<M$, and $k\in \nats$, with $k>0$:
$$
\model, x \, \models \,
\lssim{\bowtie c}{m}{M}{k}{\rho}{a}{b} \form \Leftrightarrow
\cc(h_a,h_b) \bowtie c
$$
with:\\
$h_a(i)=\mkhis(a,S(x,\rho),m,M,k)(i)$, \\
$h_b(i)=\mkhis(b,\ZET{y}{\model,y \models \form},m,M,k)(i)$,\\
$\bowtie \, \in \, \SET{=,<,>,\leq,\geq}$, and\\
$S(x,\rho)=\ZET{y\in X}{d(x,y) \leq \rho}$ is the {\em sphere} of radius $\rho$ centred in $x$. \ed
\end{definition}

So $\lssim{\bowtie c}{m}{M}{k}{\rho}{a}{b} \form$ compares the region of the space
 constituted by the sphere of radius $\rho$ centred in $x$ against the 
region characterised by $\form$. The comparison is  based on the cross correlation
of the histograms of the values of the chosen attributes of (the points of) the two regions, namely attribute $a$ for the points around $x$ and attribute $b$ for the points that satisfy $\form$. Of course, these attributes may also be chosen to be the same.
Both histograms share the same domain ($[m,M]$) and the same (number and type of) bins ($[1,k]$). The algorithm for the TA operator, and details on its complexity, can be found in~\cite{BCLM19,Ba+19}.

In summary, the operator checks {\em to which extent} the {\em sphere around the point of interest} is {\em statistically similar} to a given region (specified by) $\form$.
For example, 
$
\lssim{\geq 0.7}{200}{2000}{100}{10.0}{a}{b} \ltrue
$
is true at voxels centred in a region---of radius $10.0$---where the
distribution of the values of attribute $a$ has cross-correlation greater
than $0.7$ with the distribution of the values of attribute $b$  in the whole
image (i.e. $\form=\ltrue$). In this case, cross-correlation is computed using $100$
bins, and taking into account only attribute values between $200$ and $2000$ for both attribute $a$ and $b$.\\

%
The syntax for the TA operator in \imgqool is {\sf crossCorrelation(r,a,b,phi,m,M,k)}, where {\sf r} denotes the radius of the area taken around each point $x$, {\sf a} is the local attribute function (i.e. for points around each $x$), {\sf b} is the target attribute function for points that satisfy {\sf phi}, {\sf m} is the minimal value and {\sf M} the maximal value considered in both histograms and {\sf k} denotes the number of bins in the histograms. In the sequel we will use the same attribute, namely the intensity of pixels in the considered images, for {\sf a} and {\sf b}.

Figure~\ref{fig:TA} illustrates the operator on an image of a nevus, shown in Fig.~\ref{subfig:orig}. Assume that our task is to find all pixels that are likely to be part of the background, so healthy skin surrounding the nevus. Assume furthermore that the image is centred nicely in the middle of the image such that we can take an area close to the border as a sample of the background. We call the VoxLogicA formula that specifies this sample area $\Phi$, as shown in cyan in Fig~\ref{subfig:bgSample} as a semi-transparant overlay on the original image. Let us assume that we are interested in the intensity of the pixels. We construct the histogram $H_{\Phi}$ of the distribution of the intensity values of all the pixels that satisfy $\Phi$. Assume that $H_{\Phi}$ has $k$ bins, and a minimum and maximum value that correspond to the minimum and maximum pixel intensity in the whole image.

Next we construct the local histogram $H_x$ for each pixel $x$ in the image by taking the intensity of all the pixels that are present in a radius $rad$ around pixel $x$. This second histogram has the same number of bins and minimal and maximal values as those of histogram $H_{\Phi}$. We can now compute the similarity score for each point $x$ in the image by computing the Pearson's correlation coefficient of the histograms  $H_{\Phi}$ and $H_x$. This provides normalised values between -1 and +1. A value equal to 1 indicates perfect correlation between the histograms, a value equal to -1 indicates perfect anti-correlation. A score of value 0 indicates that there is no correlation between the histograms. The result for  Fig.~\ref{subfig:orig} is shown in Fig.~\ref{subfig:bgScore} as a semi-transparent yellow overlay where higher values of the score correspond to a brighter yellow hue. The associated histogram of these cross-correlation scores are shown in Fig.~\ref{subfig:bgSimHis}. Finally, in Fig.~\ref{subfig:bgSim}, those pixels with a cross-correlation score above 0.05 are shown as an overlay in pink.

\begin{figure}
\def\gbsz{1.9cm}
\centering
\subfloat[][]
{
\includegraphics[height=\gbsz]{img/ISIC10_nevusImgIntens_original.png}
\label{subfig:orig}
}
\centering
\subfloat[][]
{
\includegraphics[height=\gbsz]{img/ISIC10_nevusImgIntens_bgSample.png}
\label{subfig:bgSample}
}
\centering
\subfloat[][]
{
\includegraphics[height=\gbsz]{img/ISIC10_nevusImgIntens_bgSimScore.png}
\label{subfig:bgScore}
}
\centering
\subfloat[][]
{
\includegraphics[height=\gbsz]{img/ISIC10_nevusImgIntens_bgSim.png}
\label{subfig:bgSim}
}\\
\centering
\subfloat[][]
{
\includegraphics[height=\gbsz]{img/ISIC10_nevusImgIntens_original_histogram.png}
\label{subfig:origHist}
}
\centering
\subfloat[][]
{
\includegraphics[height=\gbsz]{img/ISIC10_nevusImgIntens_bgSimScore_histogram.png}
\label{subfig:bgSimHis}
}
\caption{Illustration texture analysis operator VoxLogicA. Fig.~\ref{subfig:orig} Original image of nevus (image ISIC-0000010 of the 2016 Challenge) and surrounding skin and related histogram of pixel intensity in Fig.~\ref{subfig:origHist}. Sample $\Phi$ of background pixels shown in cyan (Fig.~\ref{subfig:bgSample}). Cross-correlation score for surrounding of each pixel w.r.t. histogram of background sample $\Phi$. The score is shown in yellow. The higher the score the higher the intensity of the yellow colour of pixels in Fig.~\ref{subfig:bgScore}.  The distribution of the cross-correlation scores is shown in Fig.~\ref{subfig:bgSimHis}. Pixels with a cross-correlation score of more than 0.05 are shown in pink in Fig.~\ref{subfig:bgSim}.
}
\label{fig:TA}
\end{figure}






==> Tool.tex <==
% !TeX root = ./TACAS19.tex

\section{The Tool \imgqool}\label{sec:Tool}

%In this section we describe the tool \imgqool. 
\imgqool is a framework for image analysis, that embeds the logic \SLCSMI
into a user-oriented expression language to manipulate images. More precisely, the
\imgqool type system distinguishes
between \emph{boolean-valued} images, that can be arguments or results of the
application of \SLCSMI operators, and \emph{number-valued} images, resulting from imaging primitives.
%
Underlying such expression language is a \emph{global model checker}, that is, the set of points satisfying a logic formula is computed at once; this is done implicitly when an expression corresponding to a logic formula is saved to an image.
 %
Functionality-wise, \imgqool\ specialises \topochecker to the case of spatial analysis of {\em multi-dimensional images}. 
It interprets a specification written in the \SLCSMI language, using a set of multi-dimensional images\footnote{Besides common bitmap formats, the model loader of \imgqool\ currently supports the NIfTI (Neuro-imaging Informatics Technology Initiative) format (https://nifti.nimh.nih.gov/, version 1 and 2).
3D MR-FLAIR images in this format very often have a slice size of 256 by 256 pixels, multiplied by 20 to 30 slices.}
as models of the spatial logic, and produces as output a set of multi-dimensional images representing the valuation of user-specified expressions. For logical operators, such images are Boolean-valued, that is, \emph{regions of interest} in medical imaging terminology, which may be loaded as \emph{overlays} in medical image viewers. Non-logical operators may generate number-valued images. \imgqool augments \SLCSMI with file loading and saving primitives, and a set of additional commodity operators, specifically aimed at image analysis, that is destined to grow along with future developments of the tool.
%
The main execution modality of \imgqool is \emph{batch execution}. A (currently experimental) \emph{graphical user interface} is under development. 
\ifArx
A planned future development is \emph{interactive execution}, in particular for semi-automated analysis, by letting a domain expert calibrate numeric parameters in real-time, while seeing the intermediate and final results.
\fi

Implementation-wise, the tool achieves a two-orders-of-magnitude speedup with respect to \topochecker. Such speedup has permitted the rapid development of a novel procedure for automatic segmentation of \emph{glioblastoma} that, besides being competitive with respect to the state-of-the-art in the field (see Section \ref{sec:case-study}), is also easily \emph{replicable} and \emph{explainable} to humans, and therefore amenable of improvement by the community of medical imaging practitioners.

\subsection{Functionality}

We provide an overview of the tool functionality, starting from its syntax.
 For space reasons, we omit details on parsing rules 
%(e.g. the syntax of identifiers and infix operators, which is 
(delegated to the tool documentation).
%
In the following, \code{f, x1,\ldots, xN, x} are identifiers, 
\code{"s"} is a string, and \code{e1, \ldots, eN, e}
are expressions (to be detailed later).  A \imgqool specification consists of a text file containing a sequence of \textbf{commands} (see Specification~\ref{alg:seg} in Sect.~\ref{sec:case-study} as an example). Five commands are currently implemented:

{\small
\begin{itemize}
 \item 
 \code{let f(x1,...,xN) = e} is used for \emph{function declaration}, also in the form \code{let f = e}\emph{(constant declaration)}, and with special syntactic provisions to define \emph{infix} operators. After execution of the command, name \code{f} is bound to a function or constant that evaluates to \code{e} with the appropriate substitutions of 
 %expressions (to be detailed later) for 
 parameters;
 
 \item
 \code{load x = "s"} loads an image from file \code{"s"} and binds it to \code{x} for subsequent usage; 
 
 \item
 \code{save "s" e} stores the image resulting from evaluation of expression \code{e} to file \code{"s"};
 
 \item
 \code{print "s" e} prints to the log \ifArx (in batch mode, the console, with prints decorated by elapsed time and other debug information)\fi the string \code{s} followed by the numeric, or boolean, result of computing \code{e};
 
 \item
 \code{import "s"} imports a library of declarations from file \code{"s"}; subsequent import declarations for the \emph{same} file are not processed; furthermore, such imported files can only contain \code{let} or \code{import} commands.
\end{itemize}
}
%
\imgqool comes equipped with a set of built-in functions, such as arithmetic
operators, logic primitives as described in Section
\ref{sec:SpatialLogicFramework}, and imaging operators, for instance for
%stemming from
%basic tasks such as 
computing the gray-scale intensity of a colour image, or its colour components, or the percentiles of its values (see Section \ref{sec:specification-gbm}).
%to advanced operations such as computing
%cross correlation of histograms (see Section \ref{sec:DIASpecificOperators}). 
An
exhaustive list of the available built-ins is provided in the user
manual\footnote{See \url{https://github.com/vincenzoml/VoxLogicA}}.
%~\cite{UserManual}. 
Furthermore, a ``standard library'' is provided containing short-hands for commonly used functions, and for derived operators. 
%
An \textbf{expression} may be a numeric literal (no distinction is made between
floating point and integer constants), an identifier (e.g. \code{x}), a function
application (e.g. \code{f(x1,x2)}), an infix operator application (e.g. \code{x1
+ x2}), or a parenthesized (sub-)expression (e.g. \code{(x1 + x2)}). 


The language features \textbf{strong dynamic typing}, that is, types of expressions are unambiguously checked and errors are precisely reported, but such checks are only performed at ``run time'', that is, when evaluating closed-form expressions with no free variables. 
%Therefore, although there is no type inference, types of functions do not need to be declared. 
The type system has currently been kept lightweight (the only typing rules regard constants and function application), in order to leave the design space open to future improvements. For instance, a planned development is function and operator \emph{overloading}, as well as some form of static typing not interfering with the usability of the tool. 

However, it is \emph{not} the case that a type error may waste a long-running analysis. Type checking occurs after loading and parsing, but before analysis is run. 
%
Actual program execution after parsing is divided into two phases. First
(usually, in a negligible amount of time), all the ``save'' and ``print''
instructions are examined to determine what expressions actually \emph{need} to
be computed; in this phase, name binding is resolved, all constant and function
applications are substituted with closed expressions, types are checked and the
environment binding expressions to names is discarded. Finally, the set of
closed expressions to be evaluated is transformed into a set of tasks to be
executed, possibly in parallel, and dependencies among them. After this phase,
no further syntax processing or name resolution are needed, and it is guaranteed
that the program is free from type errors. The second phase simply runs each
task -- in an order compliant with dependencies --  parallelising execution on multiple CPU cores.

Each built-in logical operator has an associated type of its input parameters and output result. The available types are inductively defined as \code{Number}, \code{Bool}, \code{String}, \code{Model}, and \code{Valuation(t)}, where \code{t} is in turn a type. The type \code{Model} is the type assigned to \code{x} in \code{load x = "f"}; operations such as the extraction of RGB components take this type as input, and return as output the only parametric type: \code{Valuation(t)}, which is the type of a multi-dimensional image in which each voxel contains a value of type \code{t}. For instance, the red component of a loaded model has type \code{Valuation(Number)}, whereas the result of evaluating a logic formula has type \code{Valuation(Bool)}\footnote{Although such type system would permit ``odd'' types such as \code{Valuation(Model)}, there is no way to construct them; in the future this may change when appropriate.}.

\ifArx 
The design of \imgqool, and in particular its simple type system, and the low number of basic constructs, has been tailored to usability by an audience of users with diverse backgrounds. 
For example, the tool abstracts from technical aspects such as the number of bits and representation (signed/unsigned integer or floating point) of numeric values, in favour of an extremely declarative and automated approach.
In this respect, \imgqool expressions should be thought of as the equivalent, in the application domain, of SQL queries over a relational database. 
%
In this line, a very
\else
An
\fi 
 important aspect of the execution semantics of \imgqool specifications is \emph{memoization},
% In \imgqool, memoization is not just an optimization 
%technique, but rather 
constituting the core of its execution engine, and
%(see Section \ref{sec:implementation-details}), 
used to achieve maximal sharing of subformulas. In \imgqool, no expression is ever computed twice,
% \footnote{Because of memoization, \imgqool might run out-of-memory; to avoid this, on-disk caching of results is typically used (also in the tool \topochecker, based on the very same theoretical foundations); although no experiments in our case studies have ever ran out of memory, on-disk caching is obviously planned in the short-term development road-map of \imgqool.}. 
freeing the user from worrying about how many times a given function is called, and making execution of complex macros and logical operators feasible.
\ifArx % only long
A function that uses one of its parameters twice, when called with an expression \code{e} as an argument, duplicates the number of sub-expressions. In our experiments, a ten-lines-of-code definition easily generates about one million subformulas. With memoization, this reduces to the order of one hundred tasks to be executed. 
\fi % end only long



\subsection{Implementation details}\label{sec:implementation-details}

\imgqool is implemented in the functional, object-oriented programming language
\code{FSharp}, using the \code{.NET Core} implementation of the \code{.NET}
specification\footnote{See \url{https://fsharp.org} and
\url{https://dotnet.github.io}}. This permits a single code base with minimal
environment-dependent setup to be cross-compiled and deployed as a standalone
executable, for the major desktop operating systems, namely \emph{Linux},
\emph{macOS}, and \emph{Windows}. 
%
%\begin{remark} 
Despite \code{.NET} code is compiled for an intermediate machine, this does not
mean that efficiency of \imgqool is somehow ``non-native''. There are quite a
number of measures in place to maximise efficiency. First and foremost, the
execution time is heavily dominated by the time spent in native libraries (more
details below), and \imgqool\ acts as a higher-level, declarative front-end for
such libraries, adding a logical language, memoization, parallel execution, and
abstraction from a plethora of technical details that a state-of-the-art imaging
library necessarily exposes. In our experiments, parsing, memoization, and
preparation of the tasks to be run may take a fraction of a second; the rest of
the execution time (usually, several seconds, unless the analysis is extremely
simple) is spent in \emph{foreign function calls}.
%\end{remark}
%
The major performance boosters in \imgqool are: a state-of-the-art computational
imaging library (\code{ITK}); the optimised implementation of the \emph{may
reach} operator; a new algorithm for statistical cross-correlation; an efficient
memoizing execution engine; parallel evaluation of independent tasks, exploiting
modern multi-core CPUs. Moreover, special care has been put in making all
performance-critical loops \emph{allocationless}. All used memory along the
loops is pre-allocated, avoiding the risk to trigger garbage collection during
computation. We will address each of them briefly in the following.

\paragraph{ITK library.} \imgqool uses the state-of-the-art
imaging library \code{ITK}, via the \code{SimpleITK} glue
library\footnote{See \url{https://itk.org} and \url{http://www.simpleitk.org}}.
Most of the operators of \imgqool are implemented
directly by a library call. Notably, this includes the \emph{Maurer distance
transform}, used to efficently implement the distance operators of \SLCSMI.

\paragraph{Novel algorithms.} The two most relevant operators that do not have a direct implementation in \code{ITK} are \code{mayReach} and
\code{crossCorrelation}, implementing, respectively, the logical operator
$\rho$, and statistical comparison described in
Section~\ref{sec:DIASpecificOperators}. The computation of the voxels satisfying
$\slreach{\phi_1}{\phi_2}$ can be implemented either using the (classical, in
computer graphics) \emph{flood-fill} primitive, or by exploiting the
\emph{connected components} of $\phi_2$ as a reachability primitive; both
solutions are available in \code{SimpleITK}. In our experiments, connected
components perform better using this library from \code{FSharp}, for large input seeds. \ifArx %
only long
%(briefly, flooding in \code{ITK} seems to be optimized for one-voxel seeds, rather than sets of voxels).
More precisely, it is easy to see that the voxels satisfying
$\slreach{\phi_1}{\phi_2}$ are those belonging either to $\lnear \phi_1$, or to
$\lnear \psi$, where $\psi$ contains each voxel $x$ such that there is a
connected component $C$ of $\phi_2$, with $x \in C$ and $C$ containing at least
one voxel satisfying $\lnear \phi_1$. \fi % end only long 
Several
critical logical connectives (e.g. \emph{surrounded} and \emph{touch}),  are defined in terms of \code{mayReach}.
Therefore, an optimised algorithm for \code{mayReach} is a key performance
improvement. The \code{crossCorrelation} operation is resource-intensive, as it
uses the histogram of a multi-dimensional hyperrectangle at
each voxel. Pre-computation methods such as
the \emph{integral histogram}~\cite{Por05}, would not yield the expected benefits, because
cross-correlation is called only few times on the same image.
%often the case that cross-correlation is computed for different images along the same computation. 
% since the cross-correlation operator in \imgqool can be applied to images that
% are created along the computation, so these are not known
%\emph{a priori}. 
In this work, we designed a parallel algorithm
exploiting \emph{additivity} of histograms. Given two sets of values $P_1$, $P_2$, let
$h_1$, $h_2$ be their respective histograms, and let $h'_1$, $h'_2$ be the
histograms of $P_1 \setminus P_2$ and $P_2 \setminus P_1$. For $i$ a bin, we
have $h_2(i) = h_1(i) - h'_1(i) + h'_2(i)$. This property leads to a
particularly efficient algorithm when $P_1$ and $P_2$ are two hyperrectangles
centred over adjacent voxels, as $P_1 \setminus P_2$ and $P_2 \setminus P_1$ are
\emph{hyperfaces}, having one dimension less than hyperrectangles. Our
algorithm divides the image into as many partitions as the
number of available processors, and then computes a
\emph{Hamiltonian path} for each partition, passing by each of its voxels exactly once.
% After computing the histogram of a hypercube for each $h_p$ (namely the one
% centred on its first element), in parallel, 
All partitions are visited in parallel, in the
order imposed by such Hamiltonian paths; the histogram is computed incrementally as described
above; finally cross-correlation is also computed and stored in the resulting image. The {\em asymptotic algorithmic complexity} of the implementation of \SLCSMI primitives in \imgqool is linear in the number of voxels, with the exception of \code{crossCorrelation}, which, by the above explanation, has complexity $O(k\cdot n)$, where $n$ is the number of voxels, and $k$ is the size of the largest hyperface of the considered hypercube.

\paragraph{Memoizing execution semantics.} 
%As we already mentioned, no expression is computed twice in \imgqool. 
Sub-expressions in \imgqool are {\em by construction} identified up-to syntactic equality and assigned a number, representing a unique identifier (UID). UIDs start from $0$ and are contiguous, therefore admitting an array  of all existing sub-formulas to be used to pre-computed valuations of expressions without further hashing. 

%\paragraph{Dereferentiation of memory pointers.} In performance-critical functions that do not have a direct counterpart in \code{ITK}, the interoperability-oriented functionality of \code{FSharp} (and the \code{dotnet} platform) is exploited to access the underlying memory of an image directly, even with array bounds checking turned off where possible, to achieve C-like efficiency in declarative, functional code. 

\subsection{Design and data structures}

The design of \imgqool defines three implementation layers. The \emph{core} execution engine implements the concurrent, memoizing semantics of the tool. The \emph{interpreter} is responsible for translating source code into core library invocations. These two layers 
%are not yet linked to imaging libraries, and 
only include some basic arithmetic and boolean primitives.
%, with no pre-defined logical operator (not even the basic spatial operators of \SLCS). 
Operators can be added by inheriting from the abstract base class 
\ifArx
\code{Model}, which is part of the core layer, defining appropriate methods, and tagging them with the identifier and type to be used in the interpreter, using so-called \emph{\code{.NET} attributes}. Upon instantiation, all such methods are found via the \emph{reflection} capabilities of \code{FSharp}, and added to the ones available in the interpreter.
\else
\code{Model}.
\fi  
%Planned future work includes turning these first two layers into a reusable library, that can be used in other projects. 
The third implementation layer is the instantiation of the core layer to define operators from \SLCSMI, and loading and saving of graphical models, using the \code{ITK} library.  
We provide some more detail on the design of the core layer, which is the most critical part of \imgqool.
% (indeed, the imaging specific code, including \code{CrossCorrelation}, also plays a fundamental role for the algorithmic aspects of the tool, but its design is quite simple, and not affected by important design choices, such data structures and concurrency libraries/mechanisms).  
 At the time of writing, the core consists of just 350 lines of \code{FSharp} code, that has been carefully engineered not only for performance, but also for ease of maintenance and future extensions.   

The essential \textbf{classes} are  \code{ModelChecker}, \code{FormulaFactory}, \code{Formula}, and \code{Operator}, of which \code{Constant} is a subclass. Class \code{Operator} describes the available operators and their evaluation method. Class \code{Formula} is a symbolic representation of a syntactic sub-expression. Each instance of \code{Formula} has a unique numeric id (UID), an instance of \code{Operator}, and (inductively) a list of \code{Formula} instances, denoting its arguments. The UID of a formula is determined by the operator name (which is unique across the application), and the list of  parameter UIDs. Therefore, by construction, it is not possible to build two different instances of \code{Formula} that are syntactically equal.
%The class \code{FormulaFactory} manages UID assignment. It features a \code{Create} method, that given an instance of \code{Operator} and a list of UIDs, returns either a fresh instance of \code{Formula} or an existing one, using a hash table for the purpose. 
\ifArx In the current implementation, there is only one instance of \code{FormulaFactory}, but nothing prevents one to use more instances in the same program for different instances of the core layer. 
\fi
UIDs are contiguous and start from $0$. By this, all created formulas can be
inserted into an array. Furthermore, UIDs are allocated in such a way that the
natural number order is a topological sort of the dependency graph between
subformulas (that is, if $f_1$ is a parameter of $f_2$, the UID of $f_1$ is
greater than the UID of $f_2$). This is exploited in class \code{ModelChecker};
internally, the class uses an array to store the results of evaluating each
\code{Formula} instance, implementing memoization. The class \code{ModelChecker}
turns each formula into a task to be executed. Whenever a formula with UID $i$ is a parameter
of the formula with UID $j$, a dependency is noted between the
associated tasks. The high-level, lightweight concurrent programming library
\code{Hopac}\footnote{See \url{https://github.com/Hopac/Hopac}.} and its
abstractions are used to evaluate the resulting task graph, in order to maximise
CPU usage on multi-core \ifArx machines, by queuing tasks for parallel
evaluation whenever their dependencies have already been evaluated. \code{Hopac}
takes care of scheduling tasks to processor cores. This guarantees high CPU
efficiency\footnote{For instance, on the machine with 4 cores that we employ for
our tests,  we obtain about $350\%$ CPU usage or even more, depending on the
experiment (the less the dependencies, the more the efficiency). It is well
known that such kind of task scheduling is in general a hard problem, which may
be tackled more specifically in future work; however, execution times in current
applications are quite satisfactory and do not make such optimisations a high
priority task.}. The interpreter uses one instance of the class
\code{ModelChecker}, which is parameterised by one instance of \code{Model}.
\else
machines. 
\ifArx
In \imgqool, only one instance of \code{Model} is defined, namely the ``third layer'' specialised to image processing that we already mentioned.
\fi

\ifArx
\section{Experimental Evaluation:  Segmentation of Glioblastoma in 3D Medical Images}
\else
\section{Experimental Evaluation}
\fi
\label{sec:case-study}

%
%\nfm{This section is very much a preliminary draft giving an idea of how it could look like. According to me the current specification should be improved (at least finding better names for partial results and in some parts it can also be simplified I think, e.g. the definition of grow). It is not clear to me with which data we can compare ours. The BRATS 2015 paper seems a bit old, referring to 2012 and 2013. There are also proceedings of BRATS 2016, but they seem all short abstracts. This needs to be sorted out. Furthermore, I think it would be good to insert also the indexes specificity and sensitivity in the evaluation. I think Vincenzo has produced them along with the dice. Moreover, we need to give some indication of the evaluation times. }

%NEW:
The performance of \imgqool\ has been evaluated on the Brain Tumor Image
Segmentation Benchmark (BraTS) of 2017~\cite{Menze2015,Bak+17} containing 210
multi contrast MRI scans of high grade glioma patients that have been obtained from
multiple institutions and were acquired with different clinical protocols and
various scanners. All the imaging data sets provided by \brats have been
segmented manually and approved by experienced neuro-radiologists. In our
evaluation we used the T2 Fluid Attenuated Inversion Recovery (FLAIR) type
of scans, which is one of the four provided modalities in the benchmark. Use of
other modalities is planned for future work. For training, the numeric
parameters of the \imgqool specification presented in Section
\ref{sec:specification-gbm} were manually calibrated against a subset of 20
cases. Validation of the method was conducted as follows. A priori, 17 of the
210 cases can be excluded because the current procedure is not suitable for
these images. This is because of the presence of multi-focal tumours (different
tumours in different areas of the brain), or due to clearly distinguishable
artifacts in the FLAIR acquisition, or because the hyperintense area is too
large and clearly not significant (possibly by incorrect acquisition). Such
cases require further investigation. For instance, the current procedure may be
improved to identify specific types of artefacts, whereas multi-modal analysis
can be used to complement the information provided by the FLAIR image in cases
where FLAIR hyperintensity is not informative enough. In Section \ref{sec:validation}, we present
the results both for the full dataset (210 cases), and for the subset without these problematic cases (193 cases).
%contain some form of artefact in the FLAIR image or we judged our current procedure unsuitable for the exhibited pathology. 
We considered both the the {\em gross tumour volume} (GTV), corresponding to what can actually be seen on an image, and the {\em clinical target volume} (CTV) which is an extension of the GTV. For glioblastomas this margin is a 2-2.5 cm isotropic expansion of the GTV volume within the brain. 
%OLD:
%We have evaluated the performance of  \imgqool\ in two ways. The first considers the use of \imgqool\ for the segmentation of Glioblastoma in 3D medical images obtained as MRI scans in NIfTI-1 format from patients in preparation for radiotherapy. In radiotherapy the {\em clinical target volume} (CTV) of the whole tumour is considered, which is an extension of the {\em gross tumour volume} (GTV), corresponding to what can actually be seen on an image. For glioblastomas this margin is a 2-2.5 cm isotropic expansion of the GTV volume within the brain. 
%
%\ifArx % only long
%In addition, the performance of \imgqool\ has been evaluated on the Brain Tumor Image Segmentation Benchmark (BraTS) of 2017~\cite{Menze2015,Bak+17} for what concerns the GTV of the whole tumour. This evaluation provides information on the quality of the proposed approach compared to the most advanced techniques that are currently being developed.
%%The BRATS 2017 data set was made available for the Multimodal Brain Tumor Segmentation Challenge of 2017 and is therefore a very useful data set to compare our evaluation results with other state-of-the-art analysis techniques. 
%The 2017 version of this benchmark contains 211 multi contrast MRI scans of low and high grade glioma patients that have been obtained from multiple institutions and were acquired with different clinical protocols and various scanners. All the imaging data sets provided by \brats have been segmented manually and were approved by experienced neuro-radiologists. In our evaluation we have used the T2 Fluid Attenuated Inversion Recovery (FLAIR) type of scans, which is one of the four provided modalities in the benchmark. 
%%In the following we briefly describe the \SLCSMI\ specification that we used for the segmentation, illustrating (in 2D) the various intermediate phases of the segmentation procedure on a selected case study in Fig~\ref{fig:seg}. 
%\else
%In addition, the performance of \imgqool\ has been evaluated on 211 multi contrast MR scans\footnote{We have used the T2 Fluid Attenuated Inversion Recovery (FLAIR) type of scans, which is one of the four modalities provided in the benchmark. 17 of them have been excluded because they contained some form of artefacts in the FLAIR image that currently is the only type of image we consider.} of the Brain Tumor Image Segmentation Benchmark (BraTS) of 2017~\cite{Menze2015,Bak+17} for what concerns the GTV of the whole tumour. 
\ifArx
This evaluation provides information on the quality of the proposed approach compared to the most advanced techniques that are currently being developed. 
\fi 
%\fi

\subsection{\SLCSMI\ segmentation procedure}\label{sec:specification-gbm}

Specification~\ref{alg:seg} shows the tumour segmentation procedure that we used
for the evaluation\footnote{Note that, although the procedure is loosely
inspired by the one in \cite{Ba+19}, there are major differences, partly due
to a different method for identification of hyperintensities (using
percentiles), and partly since the task in this work is simpler, as we only identify the CTV and GTV (avoiding, for instance, to label the oedema).}. The syntax
is that of \imgqool, namely: \code{|,\&,!} are boolean \emph{or}, \emph{and},
\emph{not}; \code{distlt(c,phi)} is the set $\ZET{y}{\model,y \models
\dist{<c}\mathtt{phi}}$ (similarly, \code{distgeq}; distances are in
millimiters); \code{crossCorrelation(r,a,b,phi,m,M,k)} yields a cross-correlation coefficient for each voxel, to which a
predicate $c$ may be applied to obtain the \emph{statistical similarity}
function of Section \ref{sec:DIASpecificOperators}; the \code{>} operator
performs thresholding of an image; \code{border} is true on voxels that lay at
the border of the image. Operator \code{percentiles(img,mask)}, where \code{img}
is a number-valued image, and \code{mask} is boolean-valued, considers the
points identified by \code{mask}, and assigns to each such point $x$ the fraction of
points that have an intensity below that of $x$ in \code{img}.
%returns an image \code{res}, such that each voxel having attribute value $x$ in \code{img} has value $k = h/n$ in \code{res} if and only if the number of voxels that are true in \code{mask} is $n$, and among those, the ones that have value less than $x$ is $h$ (points outside of \code{mask} have value $0$ in \code{res}). 
Other operators are explained in Definition~\ref{def:derived} (see also Figure~\ref{fig:surround}).  Figure~\ref{fig:seg} shows the intermediate phases of the procedure, for axial view of one specific 2D slice of an example 3D MRI scan of the BraTS 2017 data set.
% \ifArx % only long

We briefly discuss the specification (see \cite{BCLM18arxiv} for more details). 
\ifArx
Line 1 imports the definitions of some basic derived operators. Lines 2-4 define a few specific operators for the segmentation (see Def.~\ref{def:derived}). Lines 4-5 load the 3D MRI scan in .nii format as well as the manually segmented one used for calculating the indexes. 
\else
Lines 1-8 merely define utility functions and load the image, calling it \code{flair}.
\fi
Lines 9-10 define the \code{background} as all voxels in the area of intensity less than 0.1 that touches the border of the image, and the \code{brain} as the complement of the background.
% Points that are part of the brain are all those points that do not satisfy \code{background}.
The application of \code{percentiles} in line 11 assigns to each point of the brain the percentile rank of its intensity among those that are part of \code{brain}.
 %attribute considering the range of intensities of points that are part of the brain in the FLAIR image. 
 Based on these percentiles, hyper-intense and very-intense points are identified that satisfy hI and vI, respectively (lines 12-13). Hyper-intense points have a very high likelihood to belong to tumour tissue; very-high intensity points are likely to belong to the tumour as well, or to the oedema that is usually surrounding the tumour. However, not all hyper-intense and very-intense points are part of a tumour. The idea is to identify the actual tumour using further spatial information. 
 %First of all, the hyper-intense points should form an area of certain dimensions. Moreover, they should be close to the area covered by the oedema. 
%
%Such characteristics can be easily specified in the \SLCSMI\ language. 
In lines 14-15 the hyper-intense and very-intense points are filtered, thus removing noise,
%(i.e. single points or very small areas of hyper-intense points) 
 and considering only areas of a certain relevant size. 
 The points that satisfy \code{hyperIntense} and \code{veryIntense} are shown in red in Fig.~\ref{subfig:hyper} and in Fig~\ref{subfig:very}, respectively. In line 16 the areas of hyper-intense points are extended via the \code{grow} operator, with those areas  that are very intense (possibly belonging to the oedema), and in turn touch the hyper-intense areas. The points that satisfy \code{growTum} are shown in red in Fig.~\ref{subfig:gTum}.
In line 17 the previously-defined (line 8) similarity operator is used to assign to all voxels a texture-similarity score with respect to \code{growTum}. In line 18 this operator is used to find those voxels that have a high cross correlation coefficient and thus are likely part of the tumour. The result is shown in Fig.~\ref{subfig:stat}. Finally (line 19), the voxels that are identified as part of the whole tumour are those that satisfy \code{growTum} extended with those that are statistically similar to it via the \code{grow} operator. Points that satisfy \code{tumFinal} are shown in red in Fig.~\ref{subfig:complete} and points identified by manual segmentation are shown for comparison in blue in the same figure (overlapping areas are purple).
% \fi % only long

%\enlargethispage{\baselineskip}
%\enlargethispage{\baselineskip}
%\enlargethispage{\baselineskip} 
%\enlargethispage{\baselineskip}
%\vskip -10pt

\begin{algorithm}
    \small
    \tt
\SetAlgoLined
\caption{\label{alg:seg}Full specification of tumour segmentation}
\imgImport "stdlib.imgql"\\[0.3em]
\imgLet grow(a,b) = (a \imgOr touch(b,a))\\ %was originally grow(a,b) = (a | touch(b,a)) S (!(touch(b,a)))
\imgLet flt(r,a) = distlt(r,distgeq(r,\imgNot a))\\
%\imgLet flt2(a) = distlt(2.0,distgeq(2.0,\imgNot a))\\[0.5em]
\imgLoad imgFLAIR =  "Brats17\_2013\_2\_1\_flair.nii.gz"\\ %``experiments/brats17/Brats17\_2013\_2\_1/Brats17\_2013\_2\_1\_flair.nii.gz"\\
\imgLoad imgManualSeg = "Brats17\_2013\_2\_1\_seg.nii.gz"\\ %``experiments/brats17/Brats17\_2013\_2\_1/Brats17\_2013\_2\_1\_seg.nii.gz"\\
\imgLet manualContouring = intensity(imgManualSeg) $>$ 0\\ %[0.5em]
\imgLet flair = intensity(imgFLAIR)\\
\imgLet similarFLAIRTo(a) = crossCorrelation(5,flair,flair,a,min(flair),max(flair),100)\\[0.5em]
\imgLet background = touch(flair $<$ 0.1,border)\\
\imgLet brain = \imgNot background\\
\imgLet pflair = percentiles(flair,brain)\\[0.3em] % associates points with their percentile rank
\imgLet hI = pflair $>$ 0.95\\
\imgLet vI = pflair $>$ 0.86\\
\imgLet hyperIntense = flt(5.0,hI)\\
\imgLet veryIntense =  flt(2.0,vI)\\[0.3em]
\imgLet growTum = grow(hyperIntense,veryIntense)\\
\imgLet tumSim = similarFLAIRTo(growTum)\\
\imgLet tumStatCC = flt(2.0,(tumSim $>$ 0.6))\\
%\imgLet tumTouchFLFL = (touch(tumStatFLFL,gTum)) \imgOr (touch(gTum,tumStatFLFL))\\
\imgLet tumFinal= grow(growTum,tumStatCC)\\[0.3em]
\ifArx % only long
// Compute indexes\\
\imgLet truePositives = volume(tumFinal \imgAnd manualContouring)\\
\imgLet trueNegatives = volume((\imgNot tumFinal) \imgAnd (\imgNot manualContouring))\\
\imgLet falseNegatives = volume((\imgNot tumFinal) \imgAnd manualContouring)\\
\imgLet falsePositives = volume(tumFinal \imgAnd (\imgNot manualContouring))\\
\imgLet sensitivity = truePositives / (truePositives + falseNegatives)\\
\imgLet specificity = trueNegatives / (trueNegatives + falsePositives)\\
\imgLet dice = (2 * truePositives) / ((2 * truePositives) + falseNegatives + falsePositives)\\[0.5em]
\fi
%
%// Save results\\
\imgSave "output\_Brats17\_2013\_2\_1/complete-FLAIR\_FL-seg.nii" tumFinal
\end{algorithm}

\noindent Interesting aspects of the \SLCSMI\ specification are its relative simplicity and abstraction level, fitting that of neuro-radiologists, its explainability, its time-efficient verification, admitting a rapid development cycle, and its independence of normalisation procedures through the use of percentiles rather than absolute values for the intensity of voxels.


%\begin{verbatim}
%import "stdlib.imgql"
%
%let grow(a,b) = (a | touch(b,a)) S (!(touch(b,a)))
%
%let flt5(a) = distlt(5,distgeq(5.0,!a))
%let flt2(a) = distlt(2.0,distgeq(2.0,!a))
%
%load imgFLAIR = "experiments/brats17/Brats17_2013_2_1/Brats17_2013_2_1_flair.nii.gz"
%load imgManualSeg = "experiments/brats17/Brats17_2013_2_1/Brats17_2013_2_1_seg.nii.gz"
%let manualContouring = intensity(imgManualSeg) > 0
%
%let flair = intensity(imgFLAIR)
%
%let background = touch(flair < 0.1,border)
%let brain = !background
%let pflair = percentiles(flair,brain)
%
%let hI = pflair > 0.95
%let vI = pflair > 0.86 
%
%let hyperIntense = flt5(hI)
%let veryIntense =  flt2(vI)
% 
%let gTum = grow(hyperIntense,veryIntense)
%
%let similarFLAIRTo(a) = crossCorrelation(5,flair,flair,a,min(flair),max(flair),100)
%
%let tumCCFLFL = similarFLAIRTo(gTum) 
%let tumStatFLFL = tumCCFLFL > 0.6
%
%let tumTouchFLFL = or(touch(tumStatFLFL,gTum),touch(gTum,tumStatFLFL))
%
%// Final result for tumour segmentation for radiotherapy
%let tumFLFL = grow(gTum,tumStatFLFL & distlt(15,hyperIntense))
%
%
%// Compute Dice index
%let truePositives = volume(tumFLFL & manualContouring)
%let trueNegatives = volume((!tumFLFL) & (!manualContouring))
%let falseNegatives = volume((!tumFLFL) & manualContouring)
%let falsePositives = volume(tumFLFL & (!manualContouring))
%
%let sensitivity = truePositives / (truePositives + falseNegatives)
%let specificity = trueNegatives / (trueNegatives + falsePositives)
%
%let dice = (2 * truePositives) / ((2 * truePositives) + falseNegatives + falsePositives)
%
%
%// Save results
%
%save "output_percentiles_MM_Opt4_Brats17_2013_2_1/flair.nii" flair
%save "output_percentiles_MM_Opt4_Brats17_2013_2_1/sensitivity" sensitivity
%save "output_percentiles_MM_Opt4_Brats17_2013_2_1/specificity" specificity
%save "output_percentiles_MM_Opt4_Brats17_2013_2_1/dice" dice
%save "output_percentiles_MM_Opt4_Brats17_2013_2_1/manual-contouring.nii" manualContouring
%save "output_percentiles_MM_Opt4_Brats17_2013_2_1/complete-FLAIR_FL-seg.nii" tumFLFL
%save "output_percentiles_MM_Opt4_Brats17_2013_2_1/tumStatFLFL-FLAIR_FL-seg.nii" tumStatFLFL
%save "output_percentiles_MM_Opt4_Brats17_2013_2_1/gTum-FLAIR_FL-seg.nii" gTum
%save "output_percentiles_MM_Opt4_Brats17_2013_2_1/hI-FLAIR_FL-seg.nii" hI
%save "output_percentiles_MM_Opt4_Brats17_2013_2_1/vI-FLAIR_FL-seg.nii" vI
%save "output_percentiles_MM_Opt4_Brats17_2013_2_1/hyperIntense-FLAIR_FL-seg.nii" hyperIntense
%save "output_percentiles_MM_Opt4_Brats17_2013_2_1/veryIntense-FLAIR_FL-seg.nii" veryIntense
%\end{verbatim}

\begin{figure}
\centering
\subfloat[][] %hyperIntense]
{
\includegraphics[height=2.2cm]{img/Brats17_2013_2_1_Opt4_seg/hyperIntenseAxial.png}
\label{subfig:hyper}
}\hfill
\centering
\subfloat[][] %veryIntense]
{
\includegraphics[height=2.2cm]{img/Brats17_2013_2_1_Opt4_seg/veryIntenseAxial.png}
\label{subfig:very}
}\hfill
\centering
\subfloat[][] %growTum]
{
\includegraphics[height=2.2cm]{img/Brats17_2013_2_1_Opt4_seg/gTumAxial.png}
\label{subfig:gTum}
}\hfill
\centering
\subfloat[][] %tumStatCC]
{
\includegraphics[height=2.2cm]{img/Brats17_2013_2_1_Opt4_seg/tumStatAxial.png}
\label{subfig:stat}
}\hfill
\centering
\subfloat[][]%tumFinal (red) and manual (blue)]
{
\includegraphics[height=2.2cm]{img/Brats17_2013_2_1_Opt4_seg/completeManualVLAcombinedAxial.png}
\label{subfig:complete}
}
\caption{Tumour segmentation of image {\tt Brats17\_2013\_2\_1}, FLAIR, axial 2D slice at X=155, Y=117 and Z=97. (a) hyperIntense (b) veryIntense (c) growTum (d) tumStatCC (e)  tumFinal (red) and manual (blue, overlapping area is purple).}
\label{fig:seg}
\end{figure}

\subsection{Validation results}\label{sec:validation}
%// Compute Dice index
%let truePositives = volume(tumFLFL & manualContouring)
%let trueNegatives = volume((!tumFLFL) & (!manualContouring))
%let falseNegatives = volume((!tumFLFL) & manualContouring)
%let falsePositives = volume(tumFLFL & (!manualContouring))
%
%let sensitivity = truePositives / (truePositives + falseNegatives)
%let specificity = trueNegatives / (trueNegatives + falsePositives)
%
%let dice = (2 * truePositives) / ((2 * truePositives) + falseNegatives + falsePositives)

Results of tumour segmentation are evaluated based on a number of indexes commonly used to compare the quality of different techniques (see \cite{Menze2015}). These indexes are based on the true positive (TP) voxels (voxels that are identified as part of a tumour in both manual and \imgqool\ segmentation), true negatives (TN) voxels (those that are {\em not} identified as part of a tumour in both manual and \imgqool\ segmentation), false positives (FP) voxels (those identified as part of a tumour by \imgqool\ but not by manual segmentation) and false negatives (FN) voxels (those identified as part of a tumour by manual segmentation but not by \imgqool). Based on these four types the following indexes are defined: 
\ifArx % only long
\begin{itemize}
\item sensitivity: $\mbox{TP} / (\mbox{TP} + \mbox{FN})$
\item specificity: $\mbox{TN} / (\mbox{TN} + \mbox{FP})$
\item Dice: $2*\mbox{TP} / (2*\mbox{TP} + \mbox{FN} +\mbox{FP})$
\end{itemize}
\else % only short
{\em sensitivity}: $\mbox{TP} / (\mbox{TP} + \mbox{FN})$; {\em specificity}: $\mbox{TN} / (\mbox{TN} + \mbox{FP})$; {\em Dice}: $2*\mbox{TP} / (2*\mbox{TP} + \mbox{FN} +\mbox{FP})$.
\fi
%
%\begin{itemize}
%\item sensitivity: $\mbox{TP} / (\mbox{TP} + \mbox{FN})$
%\item specificity: $\mbox{TN} / (\mbox{TN} + \mbox{FP})$
%\item Dice: $2*\mbox{TP} / (2*\mbox{TP} + \mbox{FN} +\mbox{FP})$
%\end{itemize}
%
%\ifArx % only long
Sensitivity measures the fraction of voxels that are correctly identified as part of a tumour. Specificity measures the fraction of voxels that are correctly identified as {\em not} being part of a tumour.
The Dice similarity coefficient is used to provide a measure of the similarity of two segmentations. %and ranges from 0.0 to 1.0, where 0.0 indicates that there is no overlap and 1.0 indicates a perfect overlap between the manual and \imgqool\ segmentation results. 
%\fi % end only long
%
%We considered the {\em gross tumour volume} (GTV), which corresponds to what can actually be seen on an image, and the {\em clinical target volume} (CTV). The latter contains the GTV extended with a margin for sub-clinical disease spread. For glioblastomas this margin is a 2-2.5 cm isotropic expansion of the GTV volume within the brain. 
%
Table~\ref{tab:results} shows the mean values of the above indexes both for GTV and  CTV volumes for Specification~\ref{alg:seg} applied to the BraTS 2017 training phase collection. 
% 
The top-scoring methods of the BraTS 2017 Challenge~\cite{brats17preproc} can be considered a good sample of the state-of-the-art in this domain. Among those, in order to collect significant statistics, we selected the 18 techniques that have been applied to at least 100 cases of the dataset. The {\em median} and {\em range of values} of the sensitivity, specificity and Dice indexes for the GTV segmentation of the whole tumour are, respectively, 0.88 (ranging from 0.55 to 0.97), 0.99 (0.98 to 0.999) and 0.88 (0.64 to 0.96). 
%Full data for these techniques is available in the leaderboard\footnote{\url{https://www.cbica.upenn.edu/BraTS17/lboardTraining.html} of Nov. 5, 2018}. This shows that our results are well in line with the state-of-the-art in this domain, which is very encouraging. 
The 3D images used in this experiment have size $240\times240\times155$ (about 9 million voxels). The evaluation of each case study takes about 10 seconds on \computer.

%and compares them with the results obtained among the best techniques of the BRATS 2012/2013 contest~\cite{Menze15}, where we have taken the algorithm by Zhao (I) as a reference benchmark. 
%We like to note that there are other algorithms presented in the BRATS 2012/2013 contest that were also providing good results and we refer to the full paper for a much more in-depth description and evaluation of these algorithms than we can afford for reasons of space limitations.
%
%\nfm{The BRATS paper of 2015 presents only results of BraTS 2012/2013. Are there more recent results to compare our results with?}
%
% OLD TABLE
%\begin{table}
%\begin{center}
%\begin{tabular}{| l | r | r | r | r | r | r | } \hline
%\multicolumn{4}{|c|}{\imgqool\ Mean (stdev) of 194 cases} & \multicolumn{3}{c|}{BraTS17 Mean (stdev) of 20 techniques}\\ \hline
%         & Sens. & Spec. & Dice &  Sens. & Spec. & Dice \\ \hline 
%GTV & 0,884(0,107)& 0,998(0,002)& 0,849(0,098)  &  0.846(0.120) & 0.992(0.005) & 0.850(0.095) \\ \hline
%CTV & 0,948(0,069)& 0,991(0,013)& 0,905(0,085) & N.A.& N.A.& N.A.\\ \hline
%\end{tabular}
%\end{center}
%\caption{\label{tab:results}\imgqool\ evaluation results on the BraTS 2017 benchmark. }
%\end{table}

% \begin{table}
% \begin{center}
% \begin{tabular}{| l | r | r | r | } \hline
% %\multicolumn{4}{|c|}{\imgqool\ Mean (stdev) of 193 cases} \\ \hline
%          & Sensitivity & Specificity & Dice  \\ \hline 
% GTV & 0,884(0,107)& 0,998(0,002)& 0,849(0,098)  \\ \hline
% CTV & 0,948(0,069)& 0,991(0,013)& 0,905(0,085)  \\ \hline
% \end{tabular}
% \end{center}
% \caption{\label{tab:results}\imgqool\ evaluation on 193 cases of the BraTS 2017 benchmark. }
% \end{table}
\begin{table}
    \begin{center}
    \begin{tabular}{| l | c | c | c | c | c | c | } \hline
    %\multicolumn{4}{|c|}{\imgqool\ Mean (stdev) of 193 cases} \\ \hline
             & Sensitivity & Specificity & Dice & Sensitivity & Specificity & Dice \\
             & (193 cases) & (193 cases) & (193 cases) & (210 cases) & (210 cases) & (210 cases) \\ \hline 
    GTV & 0.89(0.10)& 1.0(0.00)& 0.85(0.10) & 0.86(0.16) & 1.0(0.0)& 0.81(0.18) \\ \hline
    CTV & 0.95(0.07)& 0.99(0.01)& 0.90(0.09) & 0.93(0.14) & 0.99(0.2) & 0.87(0.15) \\ \hline
    \end{tabular}
    \end{center}
    \caption{\label{tab:results}\imgqool\ evaluation on the BraTS 2017 benchmark. }
\end{table}
    
%
% Gina 2018/10/12 using T2 to exclude some high intense areas, Mieke: spec as in this paper using only FLAIR. 17 problematic cases excluded as described
%
%dice CTV Gina	dice CTV Mieke	dice Gina GTV	dice Mieke GTV	sensitivity CTV Gina	sensitivity CTV Mieke	sensitivity Gina GTV	sensitivity Mieke GTV	specificity CTV Gina	specificity CTV Mieke	specificity Gina GTV	specificity Mieke GTV
% Mean	0,905223128	0,904720857	0,850717478	0,849224083	0,945069908	0,948139357	0,859261979	0,883791356	0,990858794	0,990527849	0,998681535	0,998303344
% STDEV	0,084138388	0,08514911	0,092041211	0,097740755	0,06946716	0,069484188	0,116364103	0,107272042	0,013190203	0,013442146	0,001409822	0,001872124
%
% Previous values
% GTV & TBD& TBD& 0.8499 (0.0936) & ca. 30s p.p. &  0.8455 (0.1204) & 0.992 (0.005) & 0.8504 (0.0947) \\ \hline
% CTV & TBD& TBD& 0.9055 (0.0836) & TBD& N.A.& N.A.& N.A.\\ \hline
%
%Table~\ref{tab:results} shows that our results are well in line with the state-of-the-art in this domain, which is very encouraging. The evaluation of each case study takes about 11 seconds, paving the way to interactive use and visualisation by neuro-radiologists, which is one of the longer term aims of our work.
%For the CTV a Dice value of 0.9 is sufficiently accurate for use in preparation of \RED{radiotherapy~\cite{Citation?}}. 
\ifArx % only long
Further inspection of results of individual cases may provide ideas for further improvements of Specification~\ref{alg:seg}.  
Furthermore, in this evaluation we have focused on the segmentation of the tumour as a whole, leaving further segmentation of the tumour in various other types of tissue (e.g. necrotic and non-enhancing parts) for future research.
\fi % end only long

%We then present the aggregated evaluation results for the whole benchmark in terms of a number of indexes that are commonly used for the assessment of the quality of a segmentation procedure. 



\subsection{Comparison with \topochecker}

%
% To get a glimpse of the sizes of data and analysis, consider that \imgqool is currently used in a case study (see Section \ref{sec:case-study}) employing sets of 3D images of size $240\times240\times155$ (about 9 millions voxels). An example specification is the one that was used in \cite{Ba+19}, which can be readily used to illustrate the performance of the tool, and to compare it with \topochecker. 
% 
% Let us first consider the involved numbers. The specification is a single, human-authored text file of about $30$ lines. The largest logic formula which is generated after expanding all macros is the one identifying the \emph{oedema}. When no sharing of sub-formulas is taken into account (that is, when execution semantics merely consists in computing each subformula when it is encountered), analysis generates $1169132$ subformulas, from a syntax tree of depth $78$. In principle, this entails over one milion of resource-intensive computational tasks to be performed.
% 
% The tool \topochecker took ... \nfv{measure times and report}.
% 
% The difference gets way more evident when considering texture analysis using cross-correlation (see Section \ref{sec:DIASpecificOperators}). \nfv{measure times for topochecker}
%
The evaluation of \imgqool that we presented in this section uses features that are present in \imgqool, but not in \topochecker.  On the other hand, the example specification in~\cite{Ba+19}, and its variant aimed at 3D images, are quite similar to the one we presented, and can be readily used to compare the performance of \imgqool and \topochecker. 
The specifications consist of two human-authored text files of about $30$ lines each. The specifications were run on \computer. In the 2D case (image size: $512 \times 512$), \topochecker took 52 seconds to complete the analysis, whereas \imgqool took 750 milliseconds. In the 3D case (image size: $512\times512\times24$), \topochecker took about 30 minutes, whereas \imgqool took 15 seconds. As we mentioned before, this huge improvement is due to the combination of a specialised imaging library, new algorithms (e.g., for statistical similarity of regions), parallel execution and other optimisations. More details could be obtained by designing a specialised set of benchmarks, where some of which can also be run using \topochecker; however, for the purposes of the current paper, the performance difference is so large that we do not deem such detailed comparison necessary. 


==> annex.tex <==


\section{Appendix}

\subsection{Foundations: Spatial Logics for Closure Spaces}
\label{sec:Kernel}
%In this section,  we  briefly introduce the notion of closure space and  the logic
%for closure spaces we use in the present paper. 
The logic for closure spaces we use in the present paper is closely related to
\SLCS~\cite{CLLM14,CLLM16} and, in particular, to the \SLCS extension with 
distance-based  operators presented in~\cite{Ba+19}. As in~\cite{Ba+19}, the resulting
logic constitutes the {\em kernel} of a solid logical framework  
for reasoning about texture features of digital %(2D, 3D, and multidimensional) 
images, when interpreted as closure spaces. 

\begin{definition}\label{def:ClosureSpaces}
A {\em closure space} is a pair $(X,\closure)$ where $X$ is a non-empty set (of {\em points})
and $\closure: 2^X \to 2^X$ is a function satisfying the following axioms:
$\closure(\emptyset)=\emptyset$;
$Y \subseteq \closure(Y)$ for all  $Y \subseteq X$;
$\closure(Y_1 \cup Y_2) = \closure(Y_1) \cup \closure(Y_2)$ for all $Y_1,Y_2\subseteq X$. \ed
\end{definition}

Given any relation $\arel \subseteq X \times X$, function $\closure_{\arel}:2^X \to 2^X$ 
with $\closure_{\arel}(Y) \triangleq Y\cup \ZET{x}{\exists y \in Y. y \, \arel \,x}$ satisfies the axioms of Definition~\ref{def:ClosureSpaces} thus making 
$(X,\closure_{\arel})$ a closure space. Whenever a closure space is generated by a relation as above, it is called a {\em quasi-discrete} closure space.
%
A quasi-discrete closure space $(X,\closure_{\arel})$, can be used as the
basis for a mathematical model of a digital image.
$X$ represents the finite set
of {\em voxels} and $\arel$ is the reflexive and symmetric  {\em adjacency} relation between voxels~\cite{Gal14}. 
\ifArx % only in long version
We note in passing that several different adjacency relations can be used.
%voxel
For instance, in the {\em orthogonal}  adjacency relation only voxels which share an edge count as adjacent, so that, in the 2D case, each pixel is adjacent  to (itself and) four other pixels; on the other hand, in the {\em orthodiagonal}  adjacency relation voxels are adjacent as long as they share at least either an edge or a corner,
so that, again in the 2D case, each pixel is adjacent  to (itself and) eight other pixels. 
\fi % end only for long
A closure space $(X,\closure)$ can be enriched with a notion of {\em distance}, i.e. a function $d: X \times X \to \reals_{\geq 0} \cup \SET{\infty}$ such that $d(x,y)=0$ iff $x=y$, leading to the {\em distance closure space} $((X,\closure),d)$.\footnote{We recall that  for 
$\emptyset\not=Y\subseteq X$, $d(x,Y) \triangleq  \inf \ZET{d(x,y)}{y \in Y}$, with $d(x,\emptyset) =\infty$.
%; note that if $Y\not=\emptyset$ is  finite, then 
%$\inf \ZET{d(x,y)}{y \in Y} = \min\ZET{d(x,y)}{y \in Y}$.
In addition, as the definition of $d$ might require the elements of $\arel$ to be weighted, 
quasi-discrete distance closure spaces
may be enriched with a $\arel$-weighting function $\weval:\arel \to \reals$
assigning the weight $\weval(x,y)$ to each $(x,y)\in \arel$. In the sequel we will keep 
$\weval$ implicit, whenever possible and for the sake of simplicity.} 

A (quasi-discrete) {\em path} $\pi$ in  $(X,\closure_{\arel})$ is a function
$\pi : \nats \to X$, 
such that for all $Y \subseteq \nats$, $\pi(\closure_{Succ}(Y)) \subseteq \closure_{\arel}(\pi(Y))$,
where  $(\nats, \closure_{Succ})$ is the closure space of natural numbers
with the {\em successor} relation: $(n,m) \in Succ \Leftrightarrow m=n+1$. Intuitively: the ordering in the path imposed by $\nats$ is compatible with relation $\arel$, i.e. $\pi(i) \, \arel\, \pi(i+1)$.
%\footnote{We refer to~\cite{CLLM16} for a discussion on paths on the more general class of closure spaces, including e.g. Euclidean spaces, including e.g. Euclidean spaces.}. 
%
%The following definition is instrumental for the definition of {\em paths}.
%
%\begin{definition}\label{def:ContFunc}
%A {\em continuous function} $f : (X_1, \closure_1) \to (X_2, \closure_2)$ is a function $f : X_1\to  X_2$
%such that, for all $Y \subseteq X_1$, we have $f(\closure_1(Y)) \subseteq \closure_2(f(Y))$.
%\ed
%\end{definition}
%
%In the definition below $(\nats, \closure_{Succ})$ is the closure space of natural numbers
%with the {\em successor} relation: $(n,m) \in Succ \Leftrightarrow m=n+1$.
%
%\begin{definition}\label{def:path}
%A (quasi-discrete) {\em path} $\pi$ in  $(X,\closure_{\arel})$ is a continuous function
%$\pi : (\nats, \closure_{Succ}) \to (X,\closure_{\arel})$.
%\ed
%\end{definition}
%We will let $\pi, \pi', \pi_1, \pi_2$ denote paths in $(X,\closure)$; the elements of $\nats$
%will be called {\em indexes} in the context of paths\footnote{We refer to~\cite{CLLM16} for a discussion on paths on the more general class of closure spaces, including e.g. Euclidean spaces, including e.g. Euclidean spaces. Here we only note that Definition~\ref{def:satisfaction} applies also to such spaces.}.
%

\ifArx
We conclude this section with an  illustration of the derived spatial operators $\mathit{touch }$, $\mathit{grow }$ and the surrounded operator in combination with the distance  
operator. In the top row of
Fig.~\ref{fig:surround} some sample input images (bitmaps) are shown of 100 by
100 points that are red, blue or black. In the second row of
Fig.~\ref{fig:surround} the results of  some spatial properties are shown, where
points in the original image that satisfy the spatial formula $\phi$ are shown
in white.
% Figure 1
Fig.~\ref{subfig:out_test3} shows the points that satisfy $\Phi=\mbox{blue } \lsurr \mbox{ red}$, i.e. blue points that are surrounded by red points in Fig.~\ref{subfig:surround_test3}. 
% Figure 2
Fig.~\ref{subfig:out_touchT4} shows the points that satisfy $\Phi=\mathit{touch}(\mbox{red},\mbox{blue})$, i.e. red points that are on a path, consisting of only red points, that reaches a blue point in Fig.~\ref{subfig:surround_test4}. There are no points that satisfy $\mathit{flt}(5.0,\mbox{red})$ as the red area has a minimal diameter which is less than 5.0 (result not shown).
%Fig.~\ref{subfig:out_test6b} shows the results for the same formula, but applied to Fig.~\ref{subfig:surround_test4} where instead no blue point is surrounded by red points. 
% Figure 3
Fig.~\ref{subfig:out_growT4} shows the points that satisfy $\Phi=\mathit{grow}(\mbox{red},\mbox{blue})$ of those in Fig.~\ref{subfig:surround_test4b}.
%Fig.~\ref{subfig:out_test5a} shows the result for $\mbox{red } \lsurr \mbox{ blue}$. Note that in this case there exist such points, because there is no way to reach black points from red points except when passing by blue points. 
% Figure 4
Fig.~\ref{subfig:out_test6c} shows the results of a formula combining the
surround operator with a distance operator where the white points are those
corresponding to red points in Fig.~\ref{subfig:surround_test6} that are
surrounded by points that are less than 11 points (in distance) away from points
that are blue. In Fig.~\ref{subfig:surround_test6} the area with red points is
30 by 30 points, the black area separating the red and the blue areas is 10
points wide. 
\else
\begin{example}\label{exa:operators}
In Figure~\ref{fig:surround}, the top row shows four pictures using colours $blue$ and $red$, interpreted as atomic propositions. Each picture in the bottom row shows in white the points that satisfy a given formula. In particular: 
Fig.~\ref{subfig:out_test3} is $blue\, \lsurr\, red$ of (a); Fig.~\ref{subfig:out_touchT4} is $\mbox{touch}(red,blue)$ of (b); Fig.~\ref{subfig:out_growT4} is $\mbox{grow}(red, blue)$ of (c); Fig.~\ref{subfig:out_test6c} is $red \, \lsurr\; ( \dist{\le 11} blue)$ of (d). 
%The examples are self-explanatory. 
For more details the reader is referred to~\cite{BCLM18arxiv}.
\end{example}
\fi % end only long

\begin{figure}
\centering
\subfloat[][]
{% Input figure 1
\includegraphics[height=1.5cm]{img/MMtest3.png}
\label{subfig:surround_test3}
}\hfill
\centering
\subfloat[][]
{% Input figure 2
\includegraphics[height=1.5cm]{img/MMtest4.png}
\label{subfig:surround_test4}
}\hfill
%\centering
%\subfloat[][Input.]
%{
%\includegraphics[height=2.0cm]{img/MMtest5.png}
%\label{subfig:surround_test5}
\centering
\subfloat[][]
{% Input figure 3
\includegraphics[height=1.5cm]{img/MMtest4.png}
\label{subfig:surround_test4b}
}\hfill
\centering
\subfloat[][]
{%Input figure 4
\includegraphics[height=1.5cm]{img/MMtest6.png}
\label{subfig:surround_test6}
}\\
\subfloat[][]%$\mbox{blue } \lsurr \mbox{ red}$ of (a).]
{% Output figure 1
\includegraphics[height=1.5cm]{img/MMtest3b_out.png}
\label{subfig:out_test3}
}\hfill
%\centering
%\subfloat[][$\mbox{blue } \lsurr \mbox{ red}$ of (b).]
%{
%\includegraphics[height=2.0cm]{img/MMtest6b_out.png}
%\label{subfig:out_test6b}
\centering
\subfloat[][]%$\mbox{touch}(\mbox{red},\mbox{blue})$ of (b).]
{% Output figure 2
\includegraphics[height=1.5cm]{img/MMtouch_rb_T4_out.png}
\label{subfig:out_touchT4}
}\hfill
%\centering
%\subfloat[][$\mbox{red } \lsurr\;  \mbox{ blue}$ of (c).]
%{
%\includegraphics[height=2.0cm]{img/MMtest5a_out.png}
%\label{subfig:out_test5a}
\centering
\subfloat[][] %$\mbox{grow}(\mbox{red},\mbox{blue})$ of (c).]
{% Output figure 3
\includegraphics[height=1.5cm]{img/MMgrowT_rb_T4_out.png}
\label{subfig:out_growT4}
}\hfill
\centering
\subfloat[][] %$\mbox{red } \lsurr\; ( \dist{\le 11} \mbox{ blue})$ of (d).]
{% Output figure 4
\includegraphics[height=1.5cm]{img/MMtest6c_out.png}
\label{subfig:out_test6c}
}
\caption{Some examples of \ImgQL operators (see Example~\ref{exa:operators}).}
\label{fig:surround}
\end{figure}

\subsection{Region similarity via statistical cross-correlation}
    %Digital Image Analysis Specific Operators}
\label{sec:DIASpecificOperators}

In the sequel, we provide some details on a logical operator, first defined in \cite{Ba+19},
that we use in the context of Texture Analysis (see for example~\cite{Kassner2010,Lopes2011,Castellano2004,Davnall2012}) 
for defining a notion of {\em statistical similarity} between image regions. 
The statistical distribution of an area $Y$ of a black and white  image is
approximated by the \emph{histogram} of the grey levels of points (voxels) 
belonging to $Y$, limiting the representation
to those levels laying in a certain interval $[m,M]$, the latter being split into $k$ {\em bins}. In the case of images modelled as closure models, where each point may have several attributes, the histogram can be defined for different attributes. Given a closure model 
$\model = ((X,\closure), \aeval, \peval)$, define function 
$\mkhis : A \times 2^X \times \reals \times \reals \times \nats \to (\nats \to \nats)$
such that for all $m<M$, $k>0$ and $i\in \SET{1,\ldots,k}$,
$
\mkhis(a,Y,m,M,k)(i) =
\Big|\ZET{y\in Y}{(i-1) \cdot \Delta \leq \aeval(y,a) - m < i \cdot\Delta}\Big|
$
where $\Delta=\frac{M-m}{k}$. 
We call $\mkhis(a,Y,m,M,k)$  the {\em histogram} of $Y$ (for attribute $a$), 
with $k$ bins and $m$, $M$ min and max values respectively.  The {\em mean}
$\mean{h}$ of a histogram  $h$ with $k$ {\em bins} is the quantity
$\frac{1}{k}\sum_{i=1}^k h(i)$. The  {\em cross correlation} between two histograms 
$h_1, h_2$  with the same number $k$ of {\em bins} is defined as follows:
$
\cc(h_1,h_2) = 
\frac
{\sum_{i=1}^k\left( h_1(i) - \mean{h_1} \right) \left(h_2(i) - \mean{h_2} \right)}
{
\sqrt{ 
\sum_{i=1}^k \left(h_1(i) - \mean{h_1} \right)^2
}
\sqrt{
\sum_{i=1}^k \left(h_2(i) - \mean{h_2} \right)^2
}
}
$.
The value of $\cc{}{}$ is \emph{normalised} so that
$-1\le \cc{}{}\le 1$; $\cc(h_1,h_2)=1$ indicates that $h_1$ and $h_2$
are \emph{perfectly correlated} (that is, $h_1 = ah_2+b$, with $a>0$); $\cc(h_1,h_2) =-1$
indicates \emph{perfect anti-correlation} (that is, $h_1=ah_2+b$, with $a<0$). On the other
hand, $\cc(h_1,h_2) = 0$ indicates no correlation. 

We embed {\em statistical similarity} $\lssim{\bowtie c}{m}{M}{k}{r}{a}{b}$ in
the logic by adding it to the grammar defined by (\ref{def:syntax}) and extending the definition of the satisfaction relation (Def.~\ref{def:satisfaction}) with the following equation,
for $m,M,k$ as above:
$$
\model, x \, \models \,
\lssim{\bowtie c}{m}{M}{k}{r}{a}{b} \form \Leftrightarrow
\cc(h_a,h_b) \bowtie c
$$
where
$h_a=\mkhis(a,S(x,r),m,M,k)$,
$h_b=\mkhis(b,\ZET{y}{\model,y \models \form},m,M,k)$,
$c$ is a constant in $[-1,1]$,
$\bowtie\, \in\SET{<, \leq, =, \geq, >}$  and
$S(x,r)=\ZET{y\in X}{d(x,y) \leq r}$ is the {\em sphere} of radius $r$ centred
in $x$. Note that, differently from \topochecker that was used in \cite{Ba+19},
in \imgqool, for efficiency reasons, $S(x,r)$ is actually the \emph{hypercube}
with edge size $2 r$, which, for anisotropic images, becomes a hyperrectangle.
So $\lssim{\bowtie c}{m}{M}{k}{r}{a}{b} \form$ compares the region of the
image constituted by the sphere (hypercube) of radius $r$ centred in $x$ against the 
region characterised by $\form$. The comparison is  based on the cross correlation
of the histograms of the chosen attributes of (the points of) the two regions, namely $a$ and $b$
and both histograms share the same range ($[m,M]$) and the same bins ($[1,k]$). 
In summary, the operator allows to check {\em to which extent} the {\em sphere (hypercube) around the point of interest} is {\em statistically similar} to a given region (specified by) $\form$.

% \RED{Finally, we introduce the {\em percentiles} operator $\prl{a}{b}{\bowtie}\; \form$ which is satisfied by a point $x$ whenever numerical attribute $b$ of $x$ is in relation $\bowtie$ with the percentile rank of numerical attribute $a$ of $x$,  w.r.t. to formula $\form$, as follows: 
% %
% $$
% \model, x \, \models \, \prl{a}{b}{\bowtie} \; \form
%  \Leftrightarrow
% \aeval(x,b) \bowtie \frac{C+0.5F}{N}
% $$
% where $C=\big| \ZET{y}{\model,y \models \form \mbox{ and } \aeval(y,a) < \aeval(x,a)} \big|$, 
% $F=\big| \ZET{y}{\model,y \models \form \mbox{ and } \aeval(y,a) = \aeval(x,a)} \big|$ and
% $N=\big|\ZET{y}{\model,y \models \form}\big|$. }
%$\mathit{percentiles}(\mathit{img},\mathit{mask})$ provides the percentile rank of a selected attribute with respect to the number of voxels that are true in $\mathit{mask}$  for each point in the mask. More formally:
%\ifArx % only long
%
%For example, a point $x$ with percentile rank 0.8 is a point in $\mathit{img}$ with an intensity such that 80\% of the points in $\mathit{img}$ that have value $\mathit{true}$ in the mask, have an intensity below that of point $p$. This quantitative operator is essential to be able to use the same segmentation specification on images that may vary in intensity distribution (i.e. a similar phenomenon as variations in slightly under or over exposed photographs). It makes it possible to avoid the use of absolute values in constraints on the intensity of points, as will be illustrated in Sect.~\ref{sec:case-study}.   
%\fi %only long
%The percentile rank of a point is defined as $pr(p)=\frac{c_l(p)+0.5*f_i(p)}{N}* 100\%$, where $c_l(p)$ is the count of all intensities that are below the intensity of $p$, $f_i(p)$ is the frequency of the intensity of $p$ and $N$ is the total number of points in the considered part of the image (namely that part corresponding to the mask). 


%\nfv{Introduce also ``percentiles'' very briefly, as another example. Mention hyperrectangles here (norm-1 hyperspheres), that we use for efficiency reasons, as otherwise the related paragraph in the implementation section makes no sense.}

